Long-Term Human Trajectory Prediction using 3D Dynamic Scene Graphs

We present a novel approach for long-term human trajectory prediction in indoor human-centric environments, which is essential for long-horizon robot planning in these environments. State-of-the-art human trajectory prediction methods are limited by their focus on collision avoidance and short-term planning, and their inability to model complex interactions of humans with the environment. In contrast, our approach overcomes these limitations by predicting sequences of human interactions with the environment and using this information to guide trajectory predictions over a horizon of up to 60s. We leverage Large Language Models (LLMs) to predict interactions with the environment by conditioning the LLM prediction on rich contextual information about the scene. This information is given as a 3D Dynamic Scene Graph that encodes the geometry, semantics, and traversability of the environment into a hierarchical representation. We then ground these interaction sequences into multi-modal spatio-temporal distributions over human positions using a probabilistic approach based on continuous-time Markov Chains. To evaluate our approach, we introduce a new semi-synthetic dataset of long-term human trajectories in complex indoor environments, which also includes annotations of human-object interactions. We show in thorough experimental evaluations that our approach achieves a 54% lower average negative log-likelihood and a 26.5% lower Best-of-20 displacement error compared to the best non-privileged (i.e., evaluated in a zero-shot fashion on the dataset) baselines for a time horizon of 60s.

==> macros.tex <==
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
%\newcommand{\todo}[1]{\blue{\textbf{(TODO: #1)}}}
% Helper commands for drafting
\NewDocumentCommand{\todo}{o m}{\textcolor{red}{\textbf{TODO\IfNoValueTF{#1}{}{(#1)}:} #2}}
\NewDocumentCommand{\note}{o m}{\textcolor{orange}{\textbf{NOTE\IfNoValueTF{#1}{}{(#1)}:} #2}}

\newcommand{\review}[1]{\blue{#1}}

\newcommand{\green}[1]{\textcolor[HTML]{026620}{#1}}
\newcommand{\CMT}[1]{\green{\textbf{(Comment: #1)}}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\LS}[1]{\red{\textbf{(LS: #1)}}}
\newcommand{\LC}[1]{\red{\textbf{(LC: #1)}}}

==> references/deprecated/newcom.tex <==
%   modifica per ottenere le lettere latine e greche in grassetto
%   sia diritte che corsive (vedi anche greche.sos)
%   BB 25-09-92
%
%   File modificato il 15/1/1993 per essere utilizzato sotto VTEX
%   accetta la definizione \pmb
%   prima di \begin{document} inserire:
%
% \renewcommand{\vet}[1]{{\pmb #1}} % ridefinizione di vet{}
% \renewcommand{\vetg}[1]{{\pmb #1}} % ridefinizione di vetg{}
%
%   modificato da BB il 16/10/2001 per introdurre una
%   definizione soddisfacente di vettore mediante {\boldsymbol } e
%   {\boldsymbol{\it }}
%
% \newcommand{\vet}[1]{{\bf #1}}
% \newcommand{\vetg}[1]{{\bf #1}}

\newcommand{\vet}[1]{{\boldsymbol {\it #1}}} % boldface in corsivo
\newcommand{\vetg}[1]{{\mathbf{ #1}}} % boldface normale
\newcommand{\quat}[1]{{\text{\texttt{\textbf{#1}}}}} % sans serif x quaternioni
\newcommand{\omoq}[1]{\tilde{{\vet{#1}}}} %
\newcommand{\omot}[1]{\tilde{{\vetg{#1}}}} %

\newcommand{\tildevet}[1]{\vet{\widetilde{#1}}} %
\newcommand{\hatvet}[1]{\vet{\widehat{{#1}}}} %
\newcommand{\barvet}[1]{\vet{\overline{{#1}}}} %

%   per i simboli di tipo blackboard (ossia quelli definiti \Mathbb)
%   dare \input{amssym1x.def} dove x vale 0 per 10pt, 1 per 11pt, 2 per 12pt

%   strutture varie

\newlength{\widthesempio}
\setlength{\widthesempio}{130mm}
\newlength{\shortesempio}
\setlength{\shortesempio}{30mm}

%\newtheorem{example}{Esempio}[section]
%\newtheorem{exercise}{Esercizio}[section]
%\newcommand{\lineaspessa}{\rule{\textwidth}{0.5mm}}

%%\theoremstyle{plain}
%\newtheorem{esempio}{$\blacksquare$ \textsf{Esempio}}[section]
%\newtheorem{example}{$\blacksquare$ \textsf{Example}}[section]
%\newtheorem{esercizio}{Esercizio}[section]

%\newcommand{\fines}{\hspace*{\fill}\rule{2.0mm}{2.0mm}}
\newcommand{\fines}{\hrulefill$\blacksquare$}

%\newtheorem{esempio}{Esempio}[section]
%\newtheorem{esercizio}{Esercizio}[section]

%   comandi abbreviati

\newcommand{\atandue}{\texttt{atan2}}
\newcommand{\Fig}[1]{\marginpar{\tt \normalsize #1}}
\newcommand{\fig}[1]{\begin{figure}[h]\vspace{#1}\end{figure}}
\newcommand{\rr}{\begin{center}\rule{\textwidth}{.5mm}\end{center}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\beq}{\protect \begin{equation}}
\newcommand{\eeq}{\protect \end{equation}}
\newcommand{\beqs}{\protect \begin{equation*}}
\newcommand{\eeqs}{\protect \end{equation*}}
%\newcommand{\bqn}{\protect \begin{equation}}
%\newcommand{\eqn}{\protect \end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\bsub}{\begin{subequations}}
\newcommand{\esub}{\end{subequations}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

% numeri immaginari/ipercomplessi

\newcommand{\ii}{\text{\sf i}}
\providecommand{\ij}{\text{\sf j}} % identico comando nel package babel
\newcommand{\ik}{\text{\sf k}}
\newcommand{\iuno}{\text{\textsf{1}}}

\newcommand{\iib}{\mathbf{i}}
\newcommand{\ijb}{\mathbf{j}}
\newcommand{\ikb}{\mathbf{k}}

\newcommand{\iivet}{\text{\bf i}}
\newcommand{\ijvet}{\text{\bf j}}
\newcommand{\geivet}{\text{\bf j}}
\newcommand{\ikvet}{\text{\bf k}}

%  quaternioni

\newcommand{\fquat}{\text{\sf f}}
\newcommand{\gquat}{\text{\sf g}}
\newcommand{\hquat}{\text{\sf h}}
\newcommand{\pquat}{\text{\sf p}}
\newcommand{\qquat}{\text{\sf q}}
\newcommand{\rquat}{\text{\sf r}}
\newcommand{\squat}{\text{\sf s}}
\newcommand{\tquat}{\text{\sf t}}
\newcommand{\uquat}{\text{\sf u}}
\newcommand{\vquat}{\text{\sf v}}
\newcommand{\wquat}{\text{\sf w}}
\newcommand{\xquat}{\text{\sf x}}
\newcommand{\yquat}{\text{\sf y}}
\newcommand{\zquat}{\text{\sf z}}

%   derivate prime

\newcommand{\adot}{\dot{a}}
\newcommand{\apunto}{\adot}

\newcommand{\bp}{\dot{b}}
\newcommand{\bdot}{\bp}
\newcommand{\bpunto}{\bp}

\newcommand{\ep}{\dot{e}}
\newcommand{\edot}{\ep}
\newcommand{\epunto}{\ep}

\newcommand{\pp}{\dot{p}}
\newcommand{\pdot}{\pp}
\newcommand{\ppunto}{\pp}

\newcommand{\qp}{\dot{q}}
\newcommand{\qdot}{\qp}
\newcommand{\qpunto}{\qp}

\newcommand{\rp}{\dot{r}}
\newcommand{\rdot}{\rp}
\newcommand{\rpunto}{\rp}

\renewcommand{\sp}{\dot{s}}
\newcommand{\sdot}{\sp}
\newcommand{\spunto}{\sp}

\newcommand{\upunto}{\dot{u}}

\newcommand{\xp}{\dot{x}}
\newcommand{\xdot}{\xp}
\newcommand{\xpunto}{\xp}

\newcommand{\yp}{\dot{y}}
\newcommand{\ydot}{\yp}
\newcommand{\ypunto}{\yp}

\newcommand{\zp}{\dot{z}}
\newcommand{\zdot}{\zp}
\newcommand{\zpunto}{\zp}

%\newcommand{\cp}{\dot{c}}
%\newcommand{\cdot}{\cp}

%   derivate seconde

\newcommand{\qpp}{\ddot{q}}
\newcommand{\qddot}{\qpp}

\newcommand{\ppp}{\ddot{p}}
\newcommand{\pddot}{\ppp}

\newcommand{\xpp}{\ddot{x}}
\newcommand{\xddot}{\xpp}

\newcommand{\spp}{\ddot{s}}
\newcommand{\sddot}{\spp}

\newcommand{\ypp}{\ddot{y}}
\newcommand{\yddot}{\ypp}

\newcommand{\epp}{\ddot{e}}
\newcommand{\eddot}{\epp}

%   lettere greche

\newcommand{\alfa}{\alpha}
\newcommand{\ro}{\rho}
\newcommand{\teta}{\theta}
\newcommand{\Teta}{\Theta}
\newcommand{\csi}{\xi}
\newcommand{\Fi}{\phi} % non usare \fi perche' e riservato a TeX
\newcommand{\lam}{\lambda}
\newcommand{\eps}{\varepsilon}
\newcommand{\ffi}{\varphi}

%   lettere calligrafiche

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

%   sistemi di riferimento

\newcommand{\Rif}[1]{{\calR}_{#1}}

% vettori con segni hat e tilde

\newcommand{\hvethat}{\hatvet{h}}
\newcommand{\hvettilde}{\tildevet{h}}
\newcommand{\Mvethat}{\hatvet{M}}
\newcommand{\Mvettilde}{\tildevet{M}}
\newcommand{\Mvetbar}{\barvet{M}}
\newcommand{\xbarvet}{\barvet{x}}
\newcommand{\xtildevet}{\tildevet{x}}

%   angoli e altro

\renewcommand{\c}{\text{c}} % quello vecchio era la cediglia
\newcommand{\s}{\text{s}}
\renewcommand{\t}{\text{t}}

\newcommand{\sfi}{\s_{\phi}}
\newcommand{\cfi}{\c_{\phi}}
\newcommand{\steta}{\s_{\theta}}
\newcommand{\cteta}{\c_{\theta}}
\newcommand{\spsi}{\s_{\psi}}
\newcommand{\cpsi}{\c_{\psi}}
\newcommand{\stx}{\s_{\theta_x}}
\newcommand{\ctx}{\c_{\theta_x}}
\newcommand{\sty}{\s_{\theta_y}}
\newcommand{\cty}{\c_{\theta_y}}
\newcommand{\stz}{\s_{\theta_z}}
\newcommand{\ctz}{\c_{\theta_z}}

%   notazioni vettoriali e matrici
%   \vet e` definito come \bf; volendo si puo` definirlo come \pmb
%   usando il comando \renewcommand{\vet}[1]{{\pmb #1}}

\newcommand{\avet}{\vet{a}}
\newcommand{\bvet}{\vet{b}}
\newcommand{\cvet}{\vet{c}}
\newcommand{\dvet}{\vet{d}}
\newcommand{\evet}{\vet{e}}
\newcommand{\fvet}{\vet{f}}
\newcommand{\gvet}{\vet{g}}
\newcommand{\hvet}{\vet{h}}
\newcommand{\ivet}{\vet{i}}
\newcommand{\jvet}{\vet{j}}
\newcommand{\kvet}{\vet{k}}
\newcommand{\lvet}{\vet{l}}
\newcommand{\ellvet}{\vet{\ell}}
\newcommand{\mvet}{\vet{m}}
\newcommand{\nvet}{\vet{n}}
\newcommand{\ovet}{\vet{o}}
\newcommand{\pvet}{\vet{p}}
\newcommand{\qvet}{\vet{q}}
\newcommand{\rvet}{\vet{r}}
\newcommand{\svet}{\vet{s}}
\newcommand{\tvet}{\vet{t}}
\newcommand{\uvet}{\vet{u}}
\newcommand{\vvet}{\vet{v}}
\newcommand{\wvet}{\vet{w}}
\newcommand{\xvet}{\vet{x}}
\newcommand{\yvet}{\vet{y}}
\newcommand{\zvet}{\vet{z}}

\newcommand{\onevet}{{\mathbf 1}}
\newcommand{\zerovet}{{\mathbf 0}}
\newcommand{\Zerovet}{\vet{O}}
\newcommand{\zeromat}{\vet{O}}

\newcommand{\Avet}{\vet{A}}
\newcommand{\Bvet}{\vet{B}}
\newcommand{\Cvet}{\vet{C}}
\newcommand{\Dvet}{\vet{D}}
\newcommand{\Evet}{\vet{E}}
\newcommand{\Fvet}{\vet{F}}
\newcommand{\Gvet}{\vet{G}}
\newcommand{\Hvet}{\vet{H}}
\newcommand{\Ivet}{\vet{I}}
\newcommand{\Jvet}{\vet{J}}
\newcommand{\Kvet}{\vet{K}}
\newcommand{\Lvet}{\vet{L}}
\newcommand{\Mvet}{\vet{M}}
\newcommand{\Nvet}{\vet{N}}
\newcommand{\Ovet}{\vet{O}}
\newcommand{\Pvet}{\vet{P}}
\newcommand{\Qvet}{\vet{Q}}
\newcommand{\Rvet}{\vet{R}}
\newcommand{\Svet}{\vet{S}}
\newcommand{\Tvet}{\vet{T}}
\newcommand{\Uvet}{\vet{U}}
\newcommand{\Vvet}{\vet{V}}
\newcommand{\Wvet}{\vet{W}}
\newcommand{\Xvet}{\vet{X}}
\newcommand{\Yvet}{\vet{Y}}
\newcommand{\Zvet}{\vet{Z}}
\newcommand{\Unovet}{\vetg{1}}

\newcommand{\pvetg}{\vetg{p}}
\newcommand{\uvetg}{\vetg{u}}
\newcommand{\vvetg}{\vetg{v}}
\newcommand{\wvetg}{\vetg{w}}
\newcommand{\xvetg}{\vetg{x}}
\newcommand{\yvetg}{\vetg{y}}
\newcommand{\zvetg}{\vetg{z}}

\newcommand{\Mvetg}{\vetg{M}}
\newcommand{\Pvetg}{\vetg{P}}
\newcommand{\Tvetg}{\vetg{T}}


% le lettere greche minuscole in grassetto possono essere dichiarate \vet

\newcommand{\alphavet}{{\vet{\alpha}}}
\newcommand{\alfavet}{{\vet{\alpha}}}
\newcommand{\betavet}{{\vet{\beta}}}
\newcommand{\gammavet}{{\vet{\gamma}}}
\newcommand{\deltavet}{{\vet{\delta}}}
\newcommand{\epsilonvet}{{\vet{\epsilon}}}
\newcommand{\zetavet}{{\vet{\zeta}}}
\newcommand{\etavet}{{\vet{\eta}}}
\newcommand{\thetavet}{{\vet{\theta}}}
\newcommand{\tetavet}{{\vet{\theta}}}
\newcommand{\iotavet}{{\vet{\iota}}}
\newcommand{\kappavet}{{\vet{\kappa}}}
\newcommand{\lambdavet}{{\vet{\lambda}}}
\newcommand{\lamvet}{{\vet{\lambda}}}
\newcommand{\muvet}{{\vet{\mu}}}
\newcommand{\nuvet}{{\vet{\nu}}}
\newcommand{\xivet}{{\vet{\xi}}}
\newcommand{\csivet}{{\vet{\xi}}}
\newcommand{\pivet}{{\vet{\pi}}}
\newcommand{\rhovet}{{\vet{\rho}}}
\newcommand{\sigmavet}{{\vet{\sigma}}}
\newcommand{\tauvet}{{\vet{\tau}}}
\newcommand{\upsilonvet}{{\vet{\upsilon}}}
\newcommand{\phivet}{{\vet{\phi}}}
\newcommand{\fivet}{{\vet{\phi}}}
\newcommand{\chivet}{{\vet{\chi}}}
\newcommand{\psivet}{{\vet{\psi}}}
\newcommand{\omegavet}{{\vet{\omega}}}
\newcommand{\varepsilonvet}{{\vet{\varepsilon}}}
\newcommand{\epsvet}{{\vet{\varepsilon}}}
\newcommand{\varthetavet}{{\vet{\vartheta}}}
\newcommand{\varphivet}{{\vet{\varphi}}}
\newcommand{\varfivet}{{\vet{\varphi}}}
\newcommand{\varpivet}{{\vet{\varpi}}}
\newcommand{\varrhovet}{{\vet{\varrho}}}
\newcommand{\varsigmavet}{{\vet{\varsigma}}}

\newcommand{\Gammavet}{\vet{\Gamma}}
\newcommand{\Gammait}{{\mathit {\Gamma}}}
\newcommand{\Deltavet}{\vet{\Delta}}
\newcommand{\Thetavet}{\vet{\Theta}}
\newcommand{\Tetavet}{\vet{\Theta}}
\newcommand{\Lambdavet}{\vet{\Lambda}}
\newcommand{\Xivet}{\vet{\Xi}}
\newcommand{\Pivet}{\vet{\Pi}}
\newcommand{\Sigmavet}{\vet{\Sigma}}
\newcommand{\Upsilonvet}{\vet{\Upsilon}}
\newcommand{\Phivet}{\vet{\Phi}}
\newcommand{\Phiit}{{\mathit {\Phi}}}
\newcommand{\Fivet}{\vet{\Phi}}
\newcommand{\Psivet}{\vet{\Psi}}
\newcommand{\Omegavet}{\vet{\Omega}}

% derivate prime

\newcommand{\alfap}{\dot{\alfa}}
\newcommand{\tetap}{\dot{\theta}}
\newcommand{\fip}{\dot{\phi}}
\newcommand{\etadot}{\dot{\eta}}
\newcommand{\csidot}{\dot{\csi}}
\newcommand{\fidot}{\dot{\phi}}
\newcommand{\lamdot}{\dot{\lambda}}
\newcommand{\pidot}{\dot{\pi}}
\newcommand{\psidot}{\dot{\psi}}
\newcommand{\tetadot}{\dot{\theta}}
\newcommand{\phidot}{\dot{\phi}}
\newcommand{\omegadot}{\dot{\omega}}
\newcommand{\omegap}{\omegadot}
\newcommand{\betadot}{\dot{\beta}}

\newcommand{\bdotvet}{\dot{\bvet}}
\newcommand{\cdotvet}{\dot{\cvet}}
\newcommand{\ddotvet}{\dot{\dvet}}
\newcommand{\edotvet}{\dot{\evet}}
\newcommand{\gdotvet}{\dot{\gvet}}
\newcommand{\pdotvet}{\dot{\pvet}}
\newcommand{\Rdotvet}{\dot{\Rvet}}
\newcommand{\rdotvet}{\dot{\rvet}}
\newcommand{\qdotvet}{\dot{\qvet}}
\newcommand{\udotvet}{\dot{\uvet}}
\newcommand{\vdotvet}{\dot{\vvet}}
\newcommand{\xdotvet}{\dot{\xvet}}
\newcommand{\ydotvet}{\dot{\yvet}}
\newcommand{\wdotvet}{\dot{\wvet}}
\newcommand{\zdotvet}{\dot{\zvet}}
\newcommand{\alfadotvet}{\dot{\alfavet}}
\newcommand{\csidotvet}{\dot{\csivet}}
\newcommand{\etadotvet}{\dot{\etavet}}
\newcommand{\tetadotvet}{\dot{\tetavet}}
\newcommand{\fidotvet}{\dot{\fivet}}
\newcommand{\omegadotvet}{\dot{\omegavet}}
\newcommand{\epsdotvet}{\dot{\epsvet}}
\newcommand{\betadotvet}{\dot{\betavet}}
\newcommand{\lambdadotvet}{\dot{\lambdavet}}
\newcommand{\lamdotvet}{\dot{\lambdavet}}
\newcommand{\xidotvet}{\dot{\xivet}}

% derivate seconde

\newcommand{\alfapp}{\ddot{\alfa}}
\newcommand{\tetapp}{\ddot{\theta}}
\newcommand{\betaddot}{\ddot{\beta}}
\newcommand{\lamddot}{\ddot{\lambda}}
\newcommand{\tetaddot}{\ddot{\theta}}

\newcommand{\bddotvet}{\ddot{\bvet}}
\newcommand{\dddotvet}{\ddot{\dvet}}
\newcommand{\eddotvet}{\ddot{\evet}}
\newcommand{\pddotvet}{\ddot{\pvet}}
\newcommand{\qddotvet}{\ddot{\qvet}}
\newcommand{\rddotvet}{\ddot{\rvet}}
\newcommand{\xddotvet}{\ddot{\xvet}}
\newcommand{\yddotvet}{\ddot{\yvet}}
\newcommand{\alfaddotvet}{\ddot{\alfavet}}
\newcommand{\csiddotvet}{\ddot{\csivet}}
\newcommand{\omegaddotvet}{\ddot{\omegavet}}
\newcommand{\betaddotvet}{\ddot{\betavet}}
\newcommand{\lamddotvet}{\ddot{\lambdavet}}

\newcommand{\Jacobian}{\vet{J}}

\newcommand{\intrip}{\int\!\!\!\!\int\!\!\!\!\int}
\newcommand{\intdop}{\int\!\!\!\!\int}

\newcommand{\rot}{\text{Rot}}
\newcommand{\trasl}{\text{Trasl}}

%\title{Le matrici di Bona}
%\author{CB}

\makeatletter
\newcommand*\setbmatrix{%
\@ifundefined{bmatrix}{%
\typeout{L'environment bmatrix non e' definito}%
\typeout{Sei sicuro di aver caricato il pacchetto amsmath?}}{%
\let\bbmatrix\bmatrix \let\endbbmatrix\endbmatrix}%
}%

\newcommand*\setpmatrix{%
\@ifundefined{pmatrix}{%
\typeout{L'environment pmatrix non e' definito}%
\typeout{Sei sicuro di aver caricato il pacchetto amsmath?}}{%
\let\bbmatrix\pmatrix \let\endbbmatrix\endpmatrix}%
}%

\newcommand*\setBmatrix{%
\@ifundefined{Bmatrix}{%
\typeout{L'environment Bmatrix non e' definito}%
\typeout{Sei sicuro di aver caricato il pacchetto amsmath?}}{%
\let\bbmatrix\Bmatrix \let\endbbmatrix\endBmatrix}%
}%

\newcommand*\setvmatrix{%
\@ifundefined{vmatrix}{%
\typeout{L'environment vmatrix non e' definito}%
\typeout{Sei sicuro di aver caricato il pacchetto amsmath?}}{%
\let\bbmatrix\vmatrix \let\endbbmatrix\endvmatrix}%
}%

\newcommand*\setVmatrix{%
\@ifundefined{Vmatrix}{%
\typeout{L'environment Vmatrix non e' definito}%
\typeout{Sei sicuro di aver caricato il pacchetto amsmath?}}{%
\let\bbmatrix\Vmatrix \let\endbbmatrix\endVmatrix}%
}%

\newcommand{\colvet}[3]{\begin{bbmatrix}#1 \\ #2 \\ #3 \end{bbmatrix}}
\newcommand{\rowvet}[3]{\begin{bbmatrix}#1 & #2 & #3 \end{bbmatrix}}

\newcommand{\omocolvet}[3]{\begin{bbmatrix}#1 \\ #2 \\ #3 \\ 1\end{bbmatrix}}
\newcommand{\omorowvet}[3]{\begin{bbmatrix}#1 & #2 & #3 & 1\end{bbmatrix}}
\newcommand{\omocolvvet}[1]{\begin{bbmatrix}#1 \\ 1\end{bbmatrix}}
\newcommand{\omorowvvet}[1]{\begin{bbmatrix}#1 & 1\end{bbmatrix}}

\newcommand{\Rot}[2]{\Rvet^{#1}_{#2}}
\newcommand{\tom}[3]{#1^{#2}_{#3}}
\newcommand{\toma}[2]{\Avet^{#1}_{#2}}
\newcommand{\tomr}[2]{\Rvet^{#1}_{#2}}
\newcommand{\tomt}[2]{\Tvet^{#1}_{#2}}
\newcommand{\Tom}[2]{
  \begin{bbmatrix}
    #1 & #2 \vspace{1ex}\\
    \zerovet\T & 1
  \end{bbmatrix}}
\newcommand{\Rotx}[1]{
  \begin{bbmatrix}
    1 &     0 &      0 \\
    0 & \c_#1 & -\s_#1 \\
    0 & \s_#1 &  \c_#1
  \end{bbmatrix}}
\newcommand{\Roty}[1]{
  \begin{bbmatrix}
    \c_#1 & 0 & \s_#1 \\
    0 & 1 &     0 \\
    -\s_#1 & 0 & \c_#1
  \end{bbmatrix}}
\newcommand{\Rotz}[1]{
  \begin{bbmatrix}
    \c_#1 & -\s_#1 & 0 \\
    \s_#1 &  \c_#1 & 0 \\
    0 &      0 & 1
  \end{bbmatrix}}
\newcommand{\Antisim}[3]{
  \begin{bbmatrix}
    0 & -#3 &  #2 \\
    #3 &   0 & -#1 \\
    -#2 &  #1 &  0
  \end{bbmatrix}}

\newcommand{\Euclid}[1]{\mathbb{E}^{#1}}
\newcommand{\eu}{{\mathrm{e}}}

%   varie

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\circa}{\approx}
\newcommand{\cov}[1]{\text{\mathrm{cov}}\left\{ #1 \right\} }
\newcommand{\conj}{^*}
\newcommand{\aster}{^{\ast}}
\newcommand{\con}[1]{#1^{\ast}}
\newcommand{\de}{{ \textrm{d}}}
\newcommand{\dep}{\partial}
%\newcommand{\defin}{\mathrel{\mathop:}=} %\newcommand{\defin}{\doteq}
%\newcommand{\defin}{\mathop:\!\!=} %\newcommand{\defin}{\doteq}
%\newcommand{\defin}{\coloneqq} %richiede package txfonts
\newcommand{\defin}{\stackrel{\text{def}}{=}}
\newcommand{\defas}{\defin}
\newcommand{\desud}[2]{\dfrac{\de #1}{\de #2}}
\newcommand{\desudt}[1]{\dfrac{\de #1}{\de t}}
\newcommand{\desudx}[1]{\dfrac{\de #1}{\de x}}
\newcommand{\depsudep}[2]{\dfrac{\dep #1}{\dep #2}}
\newcommand{\depsudepsquare}[2]{\dfrac{\dep^2 #1}{\dep #2}}
\newcommand{\diag}{\text{ diag}}
\newcommand{\e}{{ e}}
\newcommand{\expected}[1]{E \{ #1 \} }
%\newcommand{\est}{\wedge}
\newcommand{\est}{\times}
%\newcommand{\est}{\times}
\newcommand{\fracd}[2]{{\displaystyle \frac{#1}{#2}}}
\newcommand{\sumd}[2]{{\displaystyle \sum{#1}{#2}}}
\newcommand{\gradi}{^{\circ}}

\newcommand{\gei}{\text{j}} % da TOPTESI
\newcommand{\Gei}{\text{J}} % da TOPTESI
\newcommand{\inv}{^{-1}}
\newcommand{\grad}{\ifmmode {\text{grad}\;}\else{grad\;}\fi}
\newcommand{\marca}{\marginpar [$\Rightarrow$]{$\Leftarrow$}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\ohm}{\ifmmode {\Omega}\else{${\Omega}$}\fi}
\newcommand{\per}{\times}
\newcommand{\by}{\times}
\newcommand{\pscal}[2]{\left\langle #1, \; #2 \right\rangle}
\newcommand{\qm}{q^{-1}}
\newcommand{\radue}{\sqrt{2}}
\newcommand{\rom}[1]{{\text{#1}}}
\newcommand{\scr}[1]{{\text{\scriptsize #1}}}
\newcommand{\sign}{\text{sign}}
\newcommand{\T}{^{\sf T}}
%\newcommand{\T}{^{T}}
%\newcommand{\trace}[1]{\text{ tr\,}#1}
\newcommand{\trace}[1]{\text{tr\,}#1}
\newcommand{\udef}{\stackrel{def}{=}}
\newcommand{\umez}{\fracd{1}{2}}
\newcommand{\unmez}{\frac{1}{2}}
\newcommand{\pimez}{\fracd{\pi}{2}}
\newcommand{\unosu}[1]{\dfrac{1}{#1}}
\newcommand{\unsu}[1]{\frac{1}{#1}}
\newcommand{\valmed}[1]{ {\cal E} \left\{ #1 \right\} }
\newcommand{\Var}[1]{\text{Var} \{ #1 \} }


\newcommand{\rosso}[1]{{\color{red}#1}}
\newcommand{\blu}[1]{{\color{blue}#1}}
\newcommand{\rossoit}[1]{\rosso{\textit{#1}}}
\newcommand{\bluit}[1]{\blu{\textit{#1}}}


% possono dare qualche problema con il Package Babel

\providecommand{\ap}{\dot{a}} % presente in babel italian
%\providecommand{\api}[1]{^{\text{\scriptsize #1}}} % presente in babel italian
\providecommand{\api}[1]{^{\text{#1}}} % presente in babel italian
\providecommand{\ped}[1]{_{\text{#1}}} % presente in babel italian
%\renewcommand{\ped}[1]{_{\text{#1}}} % presente in babel italian
%\providecommand{\unit}[1]{\ifmmode { \, #1} % presente in babel italian
%                       \else {${ \, #1}$}
%                       \fi}
\providecommand{\unit}[1]{\ifmmode {\,\mathrm{#1}} % presente in babel italian
                       \else {${ \, #1}$}
                       \fi}
\providecommand{\rad}{\text{rad}}

%\DeclareRobustCommand*{\bbl@unit}[1]{%
%  \textormath{\,\text{#1}}{\,\mathrm{#1}}}%
%\DeclareRobustCommand*{\bbl@ap}[1]{%
%  \textormath{\textsuperscript{#1}}{^{\mathrm{#1}}}}%
%\DeclareRobustCommand*{\bbl@ped}[1]{%
%  \textormath{$_{\text{\fontshape{n}\fontsize\sf@size\z@
%          \selectfont#1}}$}{_\mathrm{#1}}}%


\newcommand{\Real}[1]{{\mathbb R}^{#1}}
\newcommand{\Complex}[1]{{\mathbb C}^{#1}}
\newcommand{\Integer}[1]{{\mathbb N}^{#1}}
\newcommand{\Rational}[1]{{\mathbb Z}^{#1}}

%\newcommand{\Real}[1]{{\mathds{R} }^{#1}} % solo con \usepackage{dsfont}
%\newcommand{\Complex}[1]{{\mathds C}^{#1}} % solo con \usepackage{dsfont}
%\newcommand{\Integer}[1]{{\mathds N}^{#1}} % solo con \usepackage{dsfont}
%\newcommand{\Rational}[1]{{\mathds Z}^{#1}} % solo con \usepackage{dsfont}

\newcommand{\preale}[1]{\text{ Re}(#1)}
\newcommand{\pimmag}[1]{\text{ Im}(#1)}

\def\qed {\hbox to \hsize {\hfill \vrule height 1.6ex width 1.5ex depth -.1ex}}

%   tipico vettore colonna 3x1

% \left[ \begin{array}{c}
% X \\
% Y \\
% Z
% \end{array} \right]

%   tipico vettore riga 1x3 trasposto

% \left[ \begin{array}{ccc}
% X & Y & Z
% \end{array} \right]

%   tipica matrice 3x3

% \begin{bmatrix}
% XXX & XXX & XXX \\
% YYY & YYY & YYY \\
% ZZZ & ZZZ & ZZZ
% \end{bmatrix}

%   tipica matrice 4x4

% \begin{bmatrix}
% XXX & XXX & XXX & XXX \\
% YYY & YYY & YYY & YYY \\
% ZZZ & ZZZ & ZZZ & ZZZ \\
% WWW & WWW & WWW & WWW
% \end{bmatrix}

%               \titolo
\newcommand{\tit}[1]{\begin{center} {\LARGE \bsf #1} \end{center}}

%               \sottotitolo
\newcommand{\sottotit}[1]{{\large \bsf #1}}

%               \esempio

%\begin{esempio}
%\label{esempio-} {
% testo esempio
%}
%\fines
%\end{esempio}

%               \esercizio

%\begin{esercizio}
%\label{es-} {
% testo esercizio
%}
%\end{esercizio}


==> references/deprecated/refManager.tex <==
%%% LONG
%% CONFERENCES
\newcommand{\ICRA}{Proc.\ of the IEEE Int.\ Conf.\ on Robotics and Automation (ICRA)}
\newcommand{\IROS}{Proc.\ of the IEEE/RSJ Int. Conf. on 
Intelligent RObots and Systems (IROS)}
\newcommand{\ISRR}{Proc.\ of the Int.\ Symposium on Robotics Research (ISRR)}
\newcommand{\RSS}{Robotics: Science and Systems (RSS)}
\newcommand{\ECMR}{Proc.\ of the European Conference on Mobile Robots (ECMR)}
\newcommand{\ICM}{Proc.\ of IEEE Int.\ Conf.\ on Mechatronics (ICM)}
\newcommand{\CDC}{Proc.\ of the IEEE Conference on Decision and Control (CDC)}
\newcommand{\ACC}{Proc.\ of the American Control Conference (ACC)}
\newcommand{\MED}{Proc.\ of the Mediterranean Conference on Control and Automation (MED)}
\newcommand{\MSC}{Proc.\ of the IEEE Multi-Conf.\ on Systems and Control (MSC)}
\newcommand{\CVPR}{Proc.\ of the Int.\ Conf.\ on Computer Vision and Pattern Recognition (CVPR)}
%
%% JOURNALS
%\newcommand{\TRO}{IEEE Trans. on Robotics}
%\newcommand{\IJRR}{Int. J. Robot. Res.}
%\newcommand{\AR}{Autonomous Robots}
%\newcommand{\JFR}{Journal of Field Robototics}
%\newcommand{\JRAS}{Robotics and Autonomous System Journal (Elsevier)}
%\newcommand{\RAM}{Robotics and Automation Magazine}
%\newcommand{\TROA}{IEEE Trans. Robot. Automat.}
%\newcommand{\TIT}{IEEE Trans. on Info. Theory}
%\newcommand{\TAC}{IEEE Transactions on Automatic Control}
%\newcommand{\SIAMopt}{SIAM J. Optim.}
%\newcommand{\SIAMcopt}{SIAM J. on Control and Optimization}
%\newcommand{\SIAMmaa}{SIAM J. Matrix Analysis Applications}
%\newcommand{\SCL}{Systems and Control Letters}
%\newcommand{\CSM}{Control Systems Magazine}
%\newcommand{\IJC}{International Journal of Control}
%\newcommand{\PIEEE}{Proc.\ of the IEEE}
%\newcommand{\TITS}{IEEE Trans. on Intelligent Transportation Systems}
%\newcommand{\TSP}{IEEE Trans. On Signal Processing}
%\newcommand{\IJCV}{Int. Journal of Computer Vision}
%\newcommand{\TPAMI}{IEEE Trans. Pattern Anal. Machine Intell.}
%\newcommand{\LNCS}{Lecture Notes in Computer Science}
%\newcommand{\AUT}{Automatica}
%\newcommand{\TSMCA}{IEEE Transactions on Systems, Man and Cybernetics, Part A}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% SHORT
% CONFERENCES
%\newcommand{\ICRA}{Int.\ Conf.\ on Robotics and Automation}
%\newcommand{\IROS}{Int.\ Conf.\ on Intelligent RObots and Systems}
%\newcommand{\RSS}{Robotics: Science and Systems}
%\newcommand{\ECMR}{European Conf.\ on Mobile Robots}
%\newcommand{\ICM}{Int.\ Conf.\ on Mechatronics}
%\newcommand{\CDC}{IEEE Conf.\ on Decision and Control}
%\newcommand{\ACC}{American Control Conf.}
%\newcommand{\MED}{Mediterranean Conf.\ on Control and Automation}
%\newcommand{\MSC}{IEEE Multi-Conf.\ on Systems and Control}
%\newcommand{\CVPR}{Int.\ Conf.\ on Computer Vision and Pattern Recognition}

% JOURNALS
\newcommand{\TRO}{IEEE Trans.\ on Robotics}
\newcommand{\IJRR}{Int.\ J.\ Robot. Res.}
\newcommand{\AR}{Autonomous Robots}
\newcommand{\JFR}{J.\ of Field Robototics}
\newcommand{\JRAS}{Robotics and Autonomous System J.}
\newcommand{\RAM}{Robotics and Automation Magazine}
\newcommand{\TROA}{IEEE Trans.\ Robot. Automat.}
\newcommand{\TIT}{IEEE Trans.\ on Info. Theory}
\newcommand{\TAC}{IEEE Trans.\ on Automatic Control}
\newcommand{\SIAMopt}{SIAM J.\ Optim.}
\newcommand{\SIAMcopt}{SIAM J.\ on Control and Optimization}
\newcommand{\SIAMmaa}{SIAM J.\ Matrix Analysis Applications}
\newcommand{\SCL}{Systems and Control Letters}
\newcommand{\CSM}{Control Systems Magazine}
\newcommand{\IJC}{Int. J.\ of Control}
\newcommand{\PIEEE}{Proc.\ of the IEEE}
\newcommand{\TITS}{IEEE Trans.\ on Intelligent Transportation Systems}
\newcommand{\TSP}{IEEE Trans.\ On Signal Processing}
\newcommand{\IJCV}{Int. J.\ of Computer Vision}
\newcommand{\TPAMI}{IEEE Trans.\ Pattern Anal. Machine Intell.}
\newcommand{\LNCS}{Lecture Notes in Computer Science}
\newcommand{\AUT}{Automatica}
\newcommand{\TSMCA}{IEEE Trans.\ on Systems, Man and Cybernetics, Part A}
\newcommand{\STAR}{Springer Tracts in Advanced Robotics}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%\newcommand{\jas}{{\it J. Atmos. Sci.}}
%\newcommand{\jpo}{{\it J. Phys. Oceanogr.}}
%\newcommand{\JPO}{{\it J. Phys. Oceanogr.}}
%\newcommand{\jfm}{{\it J. Fluid Mech.}}
%\newcommand{\jgr}{{\it J. Geophys. Res.}}
%\newcommand{\JGR}{{\it J. Geophys. Res.}}
%\newcommand{\jmr}{{\it J. Mar. Res.}}
%\newcommand{\arfm}{{\it Ann. Rev. Fluid Mech.}}
%\newcommand{\dsr}{{\it Deep-Sea Res.}}
%\newcommand{\dao}{{\it Dyn. Atmos. Oceans}}
%\newcommand{\jam}{{\it Journal of Applied Meteorology}}
%\newcommand{\phfl}{{\it Phys. Fluids}}
%\newcommand{\phfla}{{\it Phys. Fluids A}}
%\newcommand{\PhilTrans}{{\it Philosophical Transactions of the Royal Society, 
%London}}
%\newcommand{\gafd}{{\it Geophys. Astrophys. Fluid Dyn.}}
%\newcommand{\gfd}{{\it Geophys. Fluid Dyn.}}
%\newcommand{\PCE}   {{\it Physics and Chemistry of the Earth}}
%\newcommand{\PRL}   {{\it Physical Review Letters}}
%
%\newcommand{\ProgOc}{{\it Prog. Oceanography}}
%\newcommand{\WHOITR}{Woods Hole Oceanographic Institution Technical Report, WHOI-}

==> references/deprecated/refTemplates.tex <==
@article{,
	Author = {},
	Title = {},
	Journal = {},
	Volume = ,
	Number = ,
	Pages = {},
	Year = }

@inproceedings{,
	Author = {},
	Title = {},
	Booktitle = {},
	Pages = {},
	Year = }

@book{,
	Author = {},
	Title = {},
	Publisher = {},
	Year = }

==> sections/07_Ablations.tex <==
\section{Ablation Studies}
\label{sec:ablations}









%%%%%% MOVED ALL ABLATION SECTIONS TO EXPERIMENTS

\todo{arbitrary split of results and ablations -> a single results section with 6 subsections, each studying one of your questions.}
\todo{non-CTMC trajectory module is not evaluated, I think that would also be a quite interesting evaluation (otherwise we don't have any evaluation of the second module really)}
To better understand the challenge and intricacies of the novel proposed task, we conduct ablation studies to investigate the impact of different components of the task and the proposed method. 

\textbf{Temporal nature of interactions.}
A key challenge of the task is that the method has to predict not only the human's trajectory, but also the interaction times with entities in the environment. This entails a high variance of possible predictions. To give an example, a human might interact with a sink for 15\,s if they are washing their hands, but 3\,min if they are washing dishes (the action label in both cases may just be ``washing''). To investigate the impact of the temporal nature of interactions, we compare the performance of our method, when disregarding the interaction times and predicting the movement in between interactions only. As the temporal length of the predicted future trajectories is significantly shorter without the interaction times, we simply compare the average negative log-likelihood (NLL) of the predicted future trajectory. The results are shown in \cref{tab:results_nll_interaction_times}. The NLL is considerably lower when not accounting for the interaction times in the evaluation. This shows that the interactions with the environment are a key component of the task that add a lot of aleatoric uncertainty.


\begin{table}[ht]
    \begin{center}
        {\small
            \begin{tabularx}{.9\linewidth}{>{\raggedright\arraybackslash}X *{2}{>{\centering\arraybackslash}X}}
                \toprule
                & \multicolumn{2}{c}{Average NLL}\\
                \cmidrule(lr){2-3}
                 & Office & Home \\
                \midrule
                without interaction times & 4.79 & 3.06\\
                with interaction times & 6.22 & 3.66\\
                \bottomrule
            \end{tabularx}
        }
    \end{center}
    \caption{Average NLL when not accounting for interaction times in the evaluation compared to the proposed scenario with interaction times.}\label{tab:results_nll_interaction_times}
\end{table}

% show results

\textbf{Isolated performance of probabilistic trajectory prediction module.}
To test how effective the probabilistic trajectory prediction module is at inferring the spatio-temporal distribution of the human's future trajectory, we test its performance given the ground-truth future interaction entities and interaction times. This demonstrates the upper bound of the probabilistic trajectory prediction module if the prediction by the LLM was perfect. The NLL, evaluated on our dataset, given ground-truth future interaction instances or interaction semantic classes is shown in \cref{fig:results_nll_ground_truth}. This figure also validates the assumption that humans often tend to interact with close instances of a particular semantic class, as the NLL is only slightly lower when given the ground-truth interaction instances compared to when only given the ground-truth semantic classes of the entities of interaction.

\begin{figure}
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gt_interaction_ablation/nll_stats_office.png}
        \caption{performance in the office environment.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gt_interaction_ablation/nll_stats_home.png}
        \caption{performance in the home environment.}
    \end{subfigure}
    \caption{Negative log-likelihood of our method (blue), our method given the ground-truth future interaction instances (magenta) and our method given the ground-truth future interaction semantics (green, dashed). The shaded background represents one standard deviation.}
    \label{fig:results_nll_ground_truth}
\end{figure}


\textbf{Deterministic prediction vs probabilistic semantic class prediction.}
% maybe this could also be part of the method section (different flavor of the proposed method)
We compare our method to a similar, but deterministic baseline that uses a LLM to directly predict interactions with entities instance-wise instead of only predicting the semantic class of the entities. This is done to test the LLM's ability to reason about the spatial composition of the environment as well as to asses the benefits of the probabilistic formulation of the method.\todo{both versions are probabilistic, split into comparison vs deterministic prediction and comparison vs instance prediction} In contrast to the proposed method, only predicting the semantic class of the entity that the human interacts with, we assign a unique ID to each object in the environment and prompt the LLM to predict this unique ID rather than predicting the semantic class of the entity and reasoning based on proximity to infer instances.
A comparison of the performance of the two methods is shown in \cref{fig:results_nll_method_flavors}.


\begin{figure}
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/method_comparison_ablation/nll_stats_office.png}
        \caption{performance in the office environment.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/method_comparison_ablation/nll_stats_home.png}
        \caption{performance in the home environment.}
    \end{subfigure}
    \caption{Negative log-likelihood of our method (blue) and a deterministic baseline of the same structure that predicts the instance of the entity that the human interacts and models the interaction times deterministically (grey). The shaded background represents one standard deviation.}
    \label{fig:results_nll_method_flavors}
\end{figure}


\textbf{Object instance prediction vs semantic class prediction}

To evaluate our strategy of focusing on the language domain and predicting the semantic class of the object rather than the instance (ID) of the object in the environment and reasoning based on closeness, we compare our method to a similar method. In this modification of our method, each unique object is assigned an ID that is predicted 
Only predicting the semantic class proves to be more effective. This is due to the fact that \begin{enumerate*}
    \item the coverage of the interaction sequence tree is broader as for each prediction of the LLM multiple instances are accounted for. Thus, the support of the predicted distribution is greater.
    \item the human has a bias towards selecting the closest instance if their abstract goal requires them to interact with an object of a particular semantic class.
    \item the ground-truth trajectory tends to loose support completely if the predicted interaction times do not exactly match the ground-truth interaction times. This is due to the fact that the interaction times are predicted deterministically.
\end{enumerate*}

